Moments Matter:Stabilizing Policy Optimization using Return Distributions

Deep Reinforcement Learning (RL) agents often learn policies that achieve the same episodic return yet behave very differently, due to a combination of environmental (random transitions, initial conditions, reward noise) and algorithmic (minibatch selection, exploration noise) factors. In continuous control tasks, even small parameter shifts can produce unstable gaits, complicating both algorithm comparison and real-world transfer. Previous work has shown that such instability arises when policy updates traverse noisy neighborhoods and that the spread of post-update return distribution $R(\theta)$, obtained by repeatedly sampling minibatches, updating $\theta$, and measuring final returns, is a useful indicator of this noise. Although explicitly constraining the policy to maintain a narrow $R(\theta)$ can improve stability, directly estimating $R(\theta)$ is computationally expensive in high-dimensional settings. We propose an alternative that takes advantage of environmental stochasticity to mitigate update-induced variability. Specifically, we model state-action return distribution through a distributional critic and then bias the advantage function of PPO using higher-order moments (skewness and kurtosis) of this distribution. By penalizing extreme tail behaviors, our method discourages policies from entering parameter regimes prone to instability. We hypothesize that in environments where post-update critic values align poorly with post-update returns, standard PPO struggles to produce a narrow $R(\theta)$. In such cases, our moment-based correction narrows $R(\theta)$, improving stability by up to 75% in Walker2D, while preserving comparable evaluation returns.

==> Contents/Alignment-2.tex <==
\section{Stabilizing PPO with Post-Update Value Distributions}

In policy optimization algorithms such as Proximal Policy Optimization (PPO; \citealp{schulman-arxiv17a}), the critic baseline guides policy updates by estimating expected returns. 
However, each update can alter the policy in ways that introduce variability in the actual returns, which can cause the critic's estimates to misalign with the observed results. 
To address this, we propose monitoring both returns and value estimates by the critic, and then comparing their variability to assess the critic’s fidelity in tracking the true returns.

Given $N$ minibatches $\{X_i\}_{i=1}^{N}$, we generate a set of updated policy parameters 
$\{\theta_i' = U(\theta, X_i)\}_{i=1}^{N},$  where $U(\theta, X_i)$ denotes an update rule applied to the current policy parameters $\theta$ using data from minibatch $X_i$. 
For each updated policy $\theta_i'$, we evaluate its performance in the environment to obtain a return $R_i$ and, thus, create $\mathcal{R}(\theta_i')$.
We additionally record the baseline estimates of the critic $V_{\theta_i'}(s)$ for the same minibatches to form the \emph{post-update value distribution}:
$$
   \mathcal{V}(\theta) 
   \;=\; 
   \Bigl\{
       V_{\theta_i'}(s)
       \; \mid \;
       \theta_i' = U(\theta, X_i),\; s \in S
   \Bigr\}_{i=1}^N.
$$
% By comparing these two distributions, we gain insight into how well the critic aligns with the actual returns after applying each update.

\textbf{Tracking Variability for Stability.}
High variance in post-update returns indicates that policy updates produce large swings in performance, potentially undermining the reliability of advantage estimates used to guide further updates. If the critic \emph{also} exhibits a high-variance value distribution, then it closely reflects this observed volatility and can adapt more cautiously (e.g., by tighter clipping or smaller learning rates). 
In contrast, if the critic's variance remains low while the actual returns fluctuate widely, the critic’s estimates may be misleading, leading to erratic updates. Monitoring the correlation between these variances over multiple post-update distributions (rather than relying on a single snapshot) helps reveal longer-term trends and can prompt adjustments that stabilize PPO.

\begin{theorem}[Weak Alignment Causes Instability]
\label{thm:weak-alignment}
In environments where the post-update value distribution $\mathcal{V}(\theta)$ aligns weakly with the post-update return distribution $\mathcal{R}(\theta)$, the PPO algorithm is prone to erratic performance and unstable policy updates due to unreliable advantage estimates.
\end{theorem}

Mathematically, let $\sigma^2(\mathcal{R}(\theta))$ denote the variance of the post-update return distribution and $\sigma^2(\mathcal{V}(\theta))$ the variance of the post-update value distribution. When the critic accurately tracks the variability in returns, we expect these two variances to be strongly correlated:
$
   r 
   \;=\; 
   \text{Corr}\bigl(\sigma^2(\mathcal{R}(\theta)),\;\sigma^2(\mathcal{V}(\theta))\bigr)
   \;\approx\;
   1.
$
A low correlation suggests that the critic’s variance estimate is not representative of actual returns, leading to misleading advantage estimates and potentially erratic policy updates. Ensuring a high degree of alignment between these two distributions helps to maintain more stable learning dynamics in PPO.


==> Contents/Conclusion.tex <==
\section{Conclusion}
We introduce critic landscapes to enhance policy stability in RL by applying CVaR, kurtosis, and skewness penalties in PPO and SAC. Future work will expand this approach to discrete-action settings and explore adaptive penalties based on training dynamics.


==> Contents/Related-Work.tex <==
\section{Related Work}

Policy stability is a critical aspect of reinforcement learning (RL), as unstable policies can lead to erratic performance and suboptimal outcomes. Numerous studies have focused on methods to improve stability in policy optimization, often by exploring different ways to represent and manage uncertainty in RL.

\subsection{Return Landscapes in Reinforcement Learning}

The concept of \textit{return landscapes} was recently introduced to provide a visualization of return distributions as policy parameters are updated \cite{rahn_return_landscapes}. Return landscapes help in assessing the stability of a policy by examining the variability in returns after updates, allowing practitioners to identify updates that could lead to unstable policies. However, generating accurate return landscapes typically requires extensive environment interactions, making this approach computationally intensive. Our work introduces \textit{critic landscapes}, an approximation that leverages the agent's critic network to estimate return distributions efficiently.

\subsection{Conditional Value at Risk (CVaR) in RL}

Conditional Value at Risk (CVaR) is a metric often used in finance to evaluate the risk of extreme losses by focusing on the left tail of a distribution. In RL, CVaR has been applied to mitigate risk by encouraging policies that avoid low-return outcomes. Studies such as \cite{tamar_cvar_rl, chow_risk_sensitive_rl} have used CVaR to optimize policies that are robust to worst-case scenarios, particularly in high-stakes applications like autonomous driving and robotics. Our approach builds on this concept by using CVaR in combination with kurtosis and skewness to achieve more comprehensive distributional control, shaping not only the risk but also the overall stability of returns.

\subsection{Distributional Reinforcement Learning}

Distributional Reinforcement Learning (DistRL) seeks to model the full distribution of returns rather than only the expected value. Approaches such as C51 \cite{bellemare_c51} and Quantile Regression DQN \cite{dabney_qrdqn} have shown that learning the return distribution can improve policy performance and stability. These methods, however, often focus on estimating the distribution without directly controlling its shape. In contrast, our method specifically targets distributional properties like tail risk, kurtosis, and skewness, allowing us to impose stability constraints directly on the return distribution during policy optimization.

\subsection{Stabilizing PPO and SAC with Distributional Constraints}

Proximal Policy Optimization (PPO) \cite{schulman_ppo} and Soft Actor-Critic (SAC) \cite{haarnoja_sac} are popular RL algorithms known for their stability in continuous control tasks. PPO achieves stability by clipping probability ratios during updates, while SAC maximizes entropy to encourage exploration. Recent work has explored integrating risk-sensitive objectives into these algorithms \cite{risk_sensitive_ppo_sac}. Our approach, termed \textit{Landscape-PPO} and \textit{Landscape-SAC}, enhances PPO and SAC by adding critic landscape-based metrics (CVaR, kurtosis, and skewness), aiming to provide both robustness and stability in policy optimization.

\subsection{Contribution of This Work}

Our work combines insights from return landscapes, distributional RL, and risk-sensitive RL by introducing critic landscapes and a set of distributional stability metrics. By shaping the critic landscape with CVaR, kurtosis, and skewness penalties, we provide a novel framework that addresses not only extreme risks but also the overall stability of returns, contributing to more reliable policy performance in RL.



==> Contents/Tables/standard-dev.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{lccccc}
\toprule
\textbf{Environment} & \textbf{PPO} & \textbf{Post-Update-CVaR} & \textbf{DPPO} & \textbf{DPPO-Kurt (ours)} & \textbf{DPPO-Skew (ours)} \\
\midrule
Ant           & 105.51            & 89.06               & 94.03            & \textbf{77.07}    & 98.23            \\
HalfCheetah   & \textbf{264.56}   & 369.67              & 312.81           & 413.20            & 287.62           \\
Hopper        & 234.31            & 207.13              & 233.87           & \textbf{57.75}    & 142.34           \\
Walker2D      & 799.44            & 643.28              & 1246.18          & \textbf{196.06}   & 226.82           \\
\bottomrule
\end{tabular}
\caption{Standard deviation $\sigma$ of post-update return distribution for PPO, Post-Update-CVaR Rejection, DPPO, DPPO-Kurt, and DPPO-Skew across various continuous control environments. 
The values are averaged over 10 seeds, and the lowest standard deviation in each environment is highlighted.
}
\label{tab:std-dev-results}
\end{table}

==> Contents/algorithm.tex <==
\subsection{Proximal Policy Optimization (PPO)}
PPO optimizes the following objective, with clipping to prevent large updates:
\[
\mathcal{L}_{\text{PPO}} = \mathbb{E}_t \left[ \min \left( r_t(\theta) A_t, \text{clip}(r_t(\theta), 1 - \epsilon, 1 + \epsilon) A_t \right) \right],
\]
where \( r_t(\theta) \) is the probability ratio. We modify PPO by adding CVaR, kurtosis, and skewness penalties:
\[
\mathcal{L}_{\text{Landscape-PPO}} = \mathcal{L}_{\text{PPO}} + \lambda_{\text{CVaR}} \cdot \text{CVaR}_\alpha(G(\theta)) + \lambda_{\text{kurt}} \cdot \text{Kurtosis}(G(\theta)) + \lambda_{\text{skew}} \cdot |\text{Skewness}(G(\theta))|.
\]

\subsection{Soft Actor-Critic (SAC)}
SAC maximizes entropy along with expected return:
\[
\mathcal{L}_{\text{SAC}} = \mathbb{E}_t \left[ Q(s_t, a_t) - \alpha \log \pi(a_t | s_t) \right],
\]
where \( \alpha \) controls entropy. For \textbf{Landscape-SAC}, we introduce similar regularizers:
\[
\mathcal{L}_{\text{Landscape-SAC}} = \mathcal{L}_{\text{SAC}} + \lambda_{\text{CVaR}} \cdot \text{CVaR}_\alpha(G(\theta)) + \lambda_{\text{kurt}} \cdot \text{Kurtosis}(G(\theta)) + \lambda_{\text{skew}} \cdot |\text{Skewness}(G(\theta))|.
\]

